Diffusion-Based Image-to-Image Translation by Noise Correction via Prompt Interpolation

We propose a simple but effective training-free approach tailored to diffusion-based image-to-image translation. Our approach revises the original noise prediction network of a pretrained diffusion model by introducing a noise correction term. We formulate the noise correction term as the difference between two noise predictions; one is computed from the denoising network with a progressive interpolation of the source and target prompt embeddings, while the other is the noise prediction with the source prompt embedding. The final noise prediction network is given by a linear combination of the standard denoising term and the noise correction term, where the former is designed to reconstruct must-be-preserved regions while the latter aims to effectively edit regions of interest relevant to the target prompt. Our approach can be easily incorporated into existing image-to-image translation methods based on diffusion models. Extensive experiments verify that the proposed technique achieves outstanding performance with low latency and consistently improves existing frameworks when combined with them.

==> sec/Experiment__Han_Bohyung_s_conflicted_copy_2024-03-08_.tex <==
% !TEX root = ./../main.tex
\section{Experiments}
\label{sec:experiments}
In this section, we compare the proposed framework, referred to as PIC, with existing state-of-the-art training-free diffusion-based image-to-image translation methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}. 
%Then, we demonstrate that our method improves the previous frameworks when the proposed algorithm is integrated into them. 
Throughout this section, we refer to PIC-integrated algorithms as ``[Algorithm name] + PIC''.


%
\begin{table*}[t!]
	\centering
	\caption{
		Quantitative results of the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt}, Plug-and-Play~\cite{tumanyan2023plug}, and Pix2Pix-Zero~\cite{parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
		%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
		%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
		%
		% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
		%and the lower value does not imply that the algorithm achieves good performance.
		Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
	}
	\setlength\tabcolsep{2pt} 
	%\hspace{-3mm}
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\hspace{-3mm}
			\begin{tabular}{l | ccc | ccc | ccc | ccc}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{3}{c|}{PtP}
				& \multicolumn{3}{c|}{PnP}
				& \multicolumn{3}{c|}{P2P} 
				& \multicolumn{3}{c}{PIC (Ours)} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13}
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				%& CS ($\uparrow$)
				%& BD ($\downarrow$)
				%& SD ($\downarrow$)
				
				\\ 
				\cline{1-13}
				%\cline{1-16}
				
				{dog $\rightarrow$ cat}
				% & ? & ? & ?
				& \bred{0.290} & \bred{0.076} & 0.038 
				& \black{0.293} & 0.100 & \bred{0.032} 
				& 0.281 & 0.127 & 0.099
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				% & ? & ? & ?
				& \bred{0.288} & \bred{0.095} & \bred{0.042}
				& \black{0.291} & 0.099 & \black{0.033}
				& 0.282 & 0.100 & 0.054
				& \bred{0.288} & \black{0.057} & \black{0.033} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				% & ? & ? & ?
				& 0.320	& \bred{0.133}	& \bred{0.042}
				& \black{0.333}	& 0.158	& \bred{0.042}
				& 0.323	& 0.193	& 0.078
				& \bred{0.324}	& \black{0.085}	& \black{0.037} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				% & ? & ? & ?
				& 0.291	& 0.183	& 0.051
				& \black{0.299}	& \bred{0.152}	& \black{0.043}
				& 0.282	& 0.216	& 0.104
				& \bred{0.292}	& \black{0.126}	& \bred{0.050} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& \black{0.315}	& 0.147	& 0.045
				& \bred{0.314}  & \bred{0.122}	& \bred{0.039}
				& \bred{0.314}  & 0.129	& 0.046 
				& \bred{0.314}	& \black{0.085}	& \black{0.036} \\
				% & \black{0.293} & \black{0.045} & \black{0.031}\\
				
				{dog $\rightarrow$ dog w/glasses}
				& 0.310	& \bred{0.041}	& 0.020
				& 0.302	& 0.087	& 0.025 
				& \black{0.322}	& 0.050	& \black{0.015} 
				& \bred{0.312}	& \black{0.026}	& \bred{0.016} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				
				\hline
				{Average}
				& 0.302	& \bred{0.113}	& 0.040
				& \black{0.305}	& 0.120	& \bred{0.036} 
				& 0.301	& 0.136	& 0.066 
				& \bred{0.304}	& \black{0.071}	& \black{0.034} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:cmp_baselines} 
\end{table*} %TODO: Reshape this table
%

\iffalse
%
\begin{table*}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt}, Plug-and-Play~\cite{tumanyan2023plug}, and Pix2Pix-Zero~\cite{parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
		%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
		%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
		%
		% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
		%and the lower value does not imply that the algorithm achieves good performance.
		Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
	}
	%\vspace{0.1in}
	\setlength\tabcolsep{3pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\hspace{-2mm}
			\begin{tabular}{l ccc | ccc | ccc | ccc | ccc}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				\hline
				\multirow{2}{*}{Task} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{3}{c|}{DDIM}
				& \multicolumn{3}{c|}{PtP}
				& \multicolumn{3}{c|}{PnP} 
				& \multicolumn{3}{c|}{P2P}
				& \multicolumn{3}{c}{Ours} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline {14-16}
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-16}
				%\cline{1-16}
				
				{dog $\rightarrow$ cat}
				% & ? & ? & ?
				& 0.289 & 0.165 & 0.086
				& \bred{0.290} & \bred{0.076} & 0.038 
				& \black{0.293} & 0.100 & \bred{0.032} 
				& 0.281 & 0.127 & 0.099
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				% & ? & ? & ?
				& 0.282 & 0.188 & 0.089
				& \bred{0.288} & \bred{0.095} & \bred{0.042}
				& \black{0.291} & 0.099 & \black{0.033}
				& 0.282 & 0.100 & 0.054
				& \bred{0.288} & \black{0.057} & \black{0.033} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				% & ? & ? & ?
				& \bred{0.325}	& 0.299	& 0.123
				& 0.320	& \bred{0.133}	& \bred{0.042}
				& \black{0.333}	& 0.158	& \bred{0.042}
				& 0.323	& 0.193	& 0.078
				& 0.324	& \black{0.085}	& \black{0.037} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				% & ? & ? & ?
				& \bred{0.294}	& 0.301	& 0.104
				& 0.291	& 0.183	& 0.051
				& \black{0.299}	& \bred{0.152}	& \black{0.043}
				& 0.282	& 0.216	& 0.104
				& 0.292	& \black{0.126}	& \bred{0.050} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& 0.304	& 0.236	& 0.088
				& \black{0.315}	& 0.147	& 0.045
				& \bred{0.314}  & \bred{0.122}	& \bred{0.039}
				& \bred{0.314}  & 0.129	& 0.046 
				& \bred{0.314}	& \black{0.085}	& \black{0.036} \\
				% & \black{0.293} & \black{0.045} & \black{0.031}\\
				
				{dog $\rightarrow$ dog w/ glasses}
				& \bred{0.318}	& 0.137	& 0.072
				& 0.310	& \bred{0.041}	& 0.020
				& 0.302	& 0.087	& 0.025 
				& \black{0.322}	& 0.050	& \black{0.015} 
				& 0.312	& \black{0.026}	& \bred{0.016} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				
				\hline
				{Average}
				& 0.302	& 0.221	& 0.093
				& 0.302	& \bred{0.113}	& 0.040
				& \black{0.305}	& 0.120	& \bred{0.036} 
				& 0.301	& 0.136	& 0.066 
				& \bred{0.304}	& \black{0.071}	& \black{0.034} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:cmp_baselines}
\end{table*}
%
\fi
\iffalse
%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with DDIM on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pre-trained Stable Diffusion~\cite{rombach2022high} when the proposed method is integrated with Prompt-to-Prompt.
		%Plug-and-Play~\citep{tumanyan2023plug}, and Pix2Pix-Zero~\citep{parmar2023zero} on real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} using the pre-trained Stable Diffusion~\citep{rombach2022high}.  
		%Note that 
		The results of Prompt-to-Prompt are retrieved from \cref{tab:cmp_baselines}.
		Black bold-faced numbers represent better performance for each metric in each row. 
	}
	%\vspace{0.1in}
	\setlength\tabcolsep{3pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\hspace{-2mm}
			\begin{tabular}{l ccc | ccc }
				%\toprule 
				\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{DDIM}
				& \multicolumn{3}{c}{Ours}\\
				
				\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				& 0.289 & 0.165 & 0.086
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& 0.281 & 0.127 & 0.099
				%& \black{0.293} & \black{0.046} & \black{0.031} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				& 0.282 & 0.188 & 0.089
				& \black{0.288} & \black{0.057} & \black{0.033} \\
				%& 0.282 & 0.100 & 0.054
				%& \red{0.288} & \black{0.060} & \red{0.034} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				& \black{0.325}	& 0.299	& 0.123
				& 0.324	& \black{0.085}	& \black{0.037} \\
				%& 0.323	& 0.193	& 0.078
				%& \red{0.324}	& \black{0.133}	& \black{0.036} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				& \black{0.294}	& 0.301	& 0.104
				& 0.292	& \black{0.126}	& \black{0.050} \\
				%& 0.282	& 0.216	& 0.104
				%& \red{0.293}	& \black{0.086}	& \red{0.051} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& 0.304	& 0.236	& 0.088
				& \black{0.314}	& \black{0.085}	& \black{0.036} \\
				%& 0.314	& -	& 0.046 
				%& 0.314	& -	& 0.043 \\
				
				{dog $\rightarrow$ dog w/ glasses}
				& \black{0.318}	& 0.137	& 0.072
				& 0.312	& \black{0.026}	& \black{0.016} \\
				%& \black{0.322}	& 0.050	& \black{0.015} 
				%& \red{0.316}	& \black{0.037}	& 0.022 \\
				
				\hline
				{Average}
				& 0.302	& 0.221	& 0.093
				& \black{0.304}	& \black{0.071}	& \black{0.034} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	%
	\label{tab:addon_ptp}
\end{table}
%
\fi
%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pre-trained Stable Diffusion~\cite{rombach2022high} when the proposed method is integrated with Prompt-to-Prompt.
		%Plug-and-Play~\citep{tumanyan2023plug}, and Pix2Pix-Zero~\citep{parmar2023zero} on real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} using the pre-trained Stable Diffusion~\citep{rombach2022high}.  
		%Note that 
		The results of Prompt-to-Prompt are retrieved from \cref{tab:cmp_baselines}.
		Black bold-faced numbers represent better performance for each metric in each row. 
	}
	%\vspace{0.1in}
	%\vspace{-0.1in}
	\setlength\tabcolsep{8pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\hspace{-2mm}
			\begin{tabular}{l | ccc | ccc }
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{PtP}
				& \multicolumn{3}{c}{PtP + PIC (Ours)}\\
				
				%\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				& \black{0.290} & 0.076 & 0.038 
				& 0.283 & \black{0.051} & \black{0.021}  \\
				%& 0.281 & 0.127 & 0.099
				%& \black{0.293} & \black{0.046} & \black{0.031} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				& 0.288 & 0.095 & 0.042 
				& \black{0.291} & \black{0.052} & \black{0.027} \\
				%& 0.282 & 0.100 & 0.054
				%& \red{0.288} & \black{0.060} & \red{0.034} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				& \black{0.320}	& 0.133	& 0.042
				& 0.292	& \black{0.071}	& \black{0.018} \\
				%& 0.323	& 0.193	& 0.078
				%& \red{0.324}	& \black{0.133}	& \black{0.036} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				& \black{0.291}	& 0.183	& 0.051
				& 0.290	& \black{0.131}	& \black{0.034} \\
				%& 0.282	& 0.216	& 0.104
				%& \red{0.293}	& \black{0.086}	& \red{0.051} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& \black{0.315}	& 0.147	& 0.045
				& 0.301	& \black{0.070}	& \black{0.026} \\
				%& 0.314	& -	& 0.046 
				%& 0.314	& -	& 0.043 \\
				
				{dog $\rightarrow$ dog w/ glasses}
				& \black{0.310}	& 0.041	& 0.020
				& 0.301	& \black{0.038}	& \black{0.011} \\
				%& \black{0.322}	& 0.050	& \black{0.015} 
				%& \red{0.316}	& \black{0.037}	& 0.022 \\
				
				\hline
				{Average}
				& \black{0.302}	& 0.113	& 0.040
				& 0.295	& \black{0.069}	& \black{0.023} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	%
	\vspace{-1mm}
	\label{tab:addon_ptp}
\end{table}

\subsection{Implementation Details}
We develop the proposed method using the publicly available code of Pix2Pix-Zero (P2P)\footnote{\url{https://github.com/pix2pixzero/pix2pix-zero}}. 
Also, we integrate our algorithm into the previous approaches by adopting the official implementations of Prompt-to-Prompt (PtP)\footnote{\url{https://github.com/google/prompt-to-prompt}} and Plug-and-Play (PnP)\footnote{\url{https://github.com/MichalGeyer/plug-and-play}}.
To accelerate the text-driven image-to-image translation process, both the inference steps for the forward process and the denoising steps for the reverse process are reduced to $50$. 





During the forward process, we adopt Bootstrapping Language-Image Pretraining (BLIP)~\cite{li2022blip} to generate a source prompt employed as the condition of the denoising network.   
In case of the corresponding target prompt, we replace the specific words in the source prompt with alternatives depending on the assigned tasks as we mentioned in Section~\ref{subsec:text_embedding_interpolation}.
For fair comparisons, we use the same source and target prompts for all comparison algorithms during both the forward and reverse processes. 
Additionally, we adopt classifier-free guidance~\cite{ho2021classifier} following the previous methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}. 
%~\cite{parmar2023zero}. 
%In addition, we employ the official implementation codes of Prompt-to-Prompt (P2P), Plug-and-Play (PnP) 


For the implementation of the proposed method, $\tau$ and $\gamma$ are set to $25$ and $0.2$, respectively, for all experiments. 
Also, we set $\beta$ to $0.3$ for word replacement tasks (\eg dog $\rightarrow$ cat and horse $\rightarrow$ zebra) while $\beta$ is set to $0.8$ for adding phrases tasks (\eg tree $\rightarrow$ palm tree and dog $\rightarrow$ dog with glasses).
%In addition, $\tau$ is $25$

%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with Plug-and-Play~\cite{tumanyan2023plug} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pre-trained Stable Diffusion~\cite{rombach2022high} when the proposed method is integrated with Plug-and-Play.
		%Plug-and-Play~\citep{tumanyan2023plug}, and Pix2Pix-Zero~\citep{parmar2023zero} on real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} using the pre-trained Stable Diffusion~\citep{rombach2022high}. 
		%Note that 
		The results of Plug-and-Play are retrieved from \cref{tab:cmp_baselines}.
	}
	%\vspace{-0.1in}
	%\vspace{0.1in}
	\setlength\tabcolsep{8pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\hspace{-2mm}
			\begin{tabular}{l | ccc | ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{PnP}
				& \multicolumn{3}{c}{PnP + PIC (Ours)}\\
				
				%\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				%& \red{0.290} & \red{0.076} & 0.038 
				& \black{0.293} & 0.100 & 0.032  
				& 0.282 & \black{0.092} & \black{0.027} \\
				%& \black{0.293} & \black{0.046} & \black{0.031} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				%& \red{0.288} & \red{0.095} & 0.042 
				& \black{0.291} & 0.099 & 0.033 
				& 0.288 & \black{0.083} & \black{0.028} \\
				%& \red{0.288} & \black{0.060} & \red{0.034} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				%& 0.320	& \black{0.133}	& \red{0.042}
				& \black{0.333}	& 0.158	& 0.042 
				& 0.317	& \black{0.121}	& \black{0.035} \\
				%& \red{0.324}	& \black{0.133}	& \black{0.036} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				%& 0.291	& 0.183	& 0.051
				& \black{0.299}	& 0.152	& 0.043 
				& 0.285	& \black{0.135}	& \black{0.037} \\
				%& \red{0.293}	& \black{0.086}	& \red{0.051} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				%& 0.315	& -	& 0.045
				& \black{0.314}	& 0.122	& 0.039 
				& 0.295	& \black{0.070} & \black{0.024}  \\
				%& 0.314	& -	& 0.043 \\
				
				{dog $\rightarrow$ dog w/ glasses}
				%& 0.310	& \red{0.041}	& \red{0.020}
				& \black{0.302}	& 0.087	& 0.025 
				& 0.300	& \black{0.085}	& \black{0.024} \\
				%& \red{0.316}	& \black{0.037}	& 0.022 \\
				
				\hline
				{Average}
				& \black{0.305}	& 0.120	& 0.036 
				& 0.295	& \black{0.098}	& \black{0.029} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			
			
			%}
	}
	%
	\label{tab:addon_pnp}
\end{table}
%

\begin{table}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with Pix2Pix-Zero~\cite{parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pre-trained Stable Diffusion~\cite{rombach2022high} when the proposed method is integrated with Pix2Pix-Zero.
		%Plug-and-Play~\citep{tumanyan2023plug}, and Pix2Pix-Zero~\citep{parmar2023zero} on real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} using the pre-trained Stable Diffusion~\citep{rombach2022high}. 
		%Note that 
		The results of Pix2Pix-Zero are retrieved from \cref{tab:cmp_baselines}.
	}
	%\vspace{0.1in}
	%\vspace{-0.1in}
	\setlength\tabcolsep{8pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\hspace{-2mm}
			\begin{tabular}{l | ccc | ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{P2P}
				& \multicolumn{3}{c}{P2P + PIC (Ours)}\\
				
				%\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				%& \red{0.290} & \red{0.076} & 0.038 
				%& \black{0.293} & 0.100 & \red{0.032}  \\
				& 0.281 & 0.127 & 0.099
				& \black{0.282} & \black{0.051} & \black{0.017} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				%& \red{0.288} & \red{0.095} & 0.042 
				%& \black{0.291} & 0.099 & \black{0.033} \\
				& 0.282 & 0.100 & 0.054
				& \black{0.285} & \black{0.056} & \black{0.016} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				%& 0.320	& \black{0.133}	& \red{0.042}
				%& \black{0.333}	& 0.158	& \red{0.042} \\
				& \black{0.323}	& 0.193	& 0.078
				& 0.309	& \black{0.070}	& \black{0.016} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				%& 0.291	& 0.183	& 0.051
				%& \black{0.299}	& \red{0.152}	& \black{0.043} \\
				& \black{0.282}	& 0.216	& 0.104
				& 0.279	& \black{0.117}	& \black{0.017} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				%& 0.315	& -	& 0.045
				%& ?	& -	& ? \\
				& 0.314	& 0.129	& 0.046 
				& \black{0.298}	& \black{0.047}	& \black{0.014} \\
				
				{dog $\rightarrow$ dog w/ glasses}
				%& 0.310	& \red{0.041}	& \red{0.020}
				%& 0.302	& 0.087	& 0.025 \\
				& \black{0.322}	& \black{0.050}	& 0.015 
				& 0.302	& 0.053	& \black{0.011} \\
				
				
				
				\hline
				{Average}
				%& 0.310	& \red{0.041}	& \red{0.020}
				%& 0.302	& 0.087	& 0.025 \\
				& \black{0.301}	& 0.136	& 0.066 
				& 0.293	& \black{0.066}	& \black{0.015} \\
				
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	%
	\label{tab:addon_p2p}
\end{table}
%
%
\begin{figure*}[t!]
	\centering
	%\vspace{-5pt}
	%\vspace{0.2cm}
	\includegraphics[width=\linewidth]{../figures/CVPR_Comparison.pdf}
	%\vspace{-5pt}
	\caption{Qualitative comparisons between the proposed method and state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
		PIC generates target images with higher-fidelity. %compared with state-of-the-art methods. %effectively edits the region of interest while successfully preserving the background or structure of the source image. 
	}
	%Qualitative results of Pix2Pix on the Cityscapes dataset.
	% ``Output" denotes the ground-truth and ``Original" represents the uncompressed generator.}
%\vspace{0.3cm}
\label{fig:comparisons}
\end{figure*}
%
\begin{figure}
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_1_2.pdf}
	%\caption{Prompt-to-Prompt~\cite{hertz2023prompt}}
	%\label{fig:first}
\end{subfigure}
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_2_2.pdf}
	%\caption{Plug-and-Play~\cite{tumanyan2023plug}}
	%\label{fig:second}
\end{subfigure}
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_3_2.pdf}
	%\caption{Pix2Pix-Zero~\cite{parmar2023zero}}
	%\label{fig:third}
\end{subfigure}
%\vspace{3pt}
\caption{Qualitative results of existing state-of-the-art methods---(top) Prompt-to-Prompt~\cite{hertz2023prompt}, (middle) Plug-and-Play~\cite{tumanyan2023plug}, and (bottom) Pix2Pix-Zero~\cite{parmar2023zero}---and their integrations with the proposed method on data sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
	%The proposed method is effective to preserve the structure or background when combined with the previous frameworks.
}
%Prompt-to-Prompt~\cite{}, Plug-and-Play~\cite{}, Pix2Pix-Zero~\cite{}, and }
\label{fig:addon}
\end{figure}


\subsection{Evaluation Metrics}
For quantitative evaluations, we measure CLIP Similarity~\cite{hessel2021clipscore}, Background Distance, and Structure Distance~\cite{tumanyan2022splicing} following Pix2Pix-Zero~\cite{parmar2023zero}. 
To evaluate the metrics, we choose $250$ images deemed most relevant to a given task by calculating the cosine similarity between the CLIP image embedding and CLIP text embedding of the source task.
CLIP similarity~\cite{hessel2021clipscore} quantifies how well the translated images are aligned with the target prompts.
To this end, we measure the cosine similarity between two CLIP embeddings of the target images and target prompts. 
On the other hand, background distance calculates the Learned Perceptual Image Patch Similarity (LPIPS) score~\cite{zhang2018unreasonable} between the background regions of the source and target images.
In order to estimate the background region, we employ the prediction of the pretrained object detector~\cite{zhou2022detecting}. 
%Lower values of the background distance suggest that the background regions of the source images are better preserved in the translated results. 
Also, structure distance~\cite{tumanyan2022splicing} is employed to evaluate the structural difference between the source and translated images. 
It computes the Frobenius norm between two self-attention maps given by the DINO-ViT network output~\cite{caron2021emerging} using the source and translated results as inputs, respectively. 
%Lower structure distance values imply that the translation images more effectively maintains the structure in the source images.


%\paragraph{CLIP Similarity (CS)}
%CLIP similarity~\cite{hessel2021clipscore} quantifies how well the translated images are aligned with the target prompts.
%To this end, we measure the cosine similarity between two CLIP embeddings of the target images and target prompts. 
%given by the pretrained CLIP image encoder and text encoder, respectively.  
%The higher CLIP similarity implies that 





%\subsubsection{Background Distance (BD)}
%\paragraph{Background Distance (BD)} 
%Background distance calculates the Learned Perceptual Image Patch Similarity (LPIPS) score~\cite{zhang2018unreasonable} between the background regions of the source and target images.
%In order to estimate the background region, we employ the prediction of the pretreined object detector~\cite{zhou2022detecting}. 
%Lower values of the background distance suggest that the background regions of the source images are better preserved in the translated results. 





%\subsubsection{Structure Distance (SD)}
%\paragraph{Structure Distance (SD)}
%Structure distance~\cite{tumanyan2022splicing} is employed to evaluate the structural difference between the source and translated images. 
%It computes the Frobenius norm between two self-attention maps given by the DINO-ViT network output~\cite{caron2021emerging} using the source and translated results as inputs, %respectively. 
%Lower structure distance values imply that the translation images more effectively maintains the structure in the source images.








\iffalse
%
\begin{figure*}[t!]
\centering
%\vspace{-5pt}
%\vspace{0.2cm}
\includegraphics[width=0.90\linewidth]{../figures/CVPR_Addon.pdf}
%\vspace{-5pt}
\caption{\ms{TODO TODO TODO}}
%Qualitative results of Pix2Pix on the Cityscapes dataset.
% ``Output" denotes the ground-truth and ``Original" represents the uncompressed generator.}
%\vspace{0.3cm}
\label{fig:comparisons}
\end{figure*}
%
\fi




\iffalse
%
\begin{table*}[t!]
\centering
\caption{
Ablation study results on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
%
% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
%and the lower value does not imply that the algorithm achieves good performance.
%Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
}
%\vspace{0.1in}
\setlength\tabcolsep{3pt} 
\scalebox{0.80}{
%\resizebox{\linewidth}{!}{
\hspace{-2mm}
\begin{tabular}{l ccc ccc ccc}
	%\toprule 
	\hline
	\multirow{2}{*}{Task} 
	& \multicolumn{3}{c}{DDIM}
	& \multicolumn{3}{c}{Prompt Interpolation}
	%& \multicolumn{3}{c}{P2P} 
	& \multicolumn{3}{c}{Ours} \\
	
	\cline{2-4} \cline{5-7} \cline{8-10} %\cline{11-13}
	
	& CS ($\uparrow$)
	& BD ($\downarrow$)
	& SD ($\downarrow$)
	
	
	& CS ($\uparrow$)
	& BD ($\downarrow$)
	& SD ($\downarrow$)
	
	& CS ($\uparrow$)
	& BD ($\downarrow$)
	& SD ($\downarrow$)
	
	
	
	
	\\ 
	\cline{1-10}
	
	{dog $\rightarrow$ cat}
	& ? & ? & ? 
	& ? & ? & ? 
	%& 0.281 & 0.127 & 0.099
	& \black{0.293} & \black{0.045} & \black{0.031} \\
	
	
	
	
	
	
	
	{cat $\rightarrow$ dog}
	& ? & ? & ?
	& ? & ? & ?
	%& 0.282 & 0.100 & 0.054
	& \bred{0.288} & \black{0.057} & \black{0.033} \\
	
	
	
	
	
	{horse $\rightarrow$ zebra}
	& ?	& ?	& ?
	& ?	& ?	& ?
	%& 0.323	& 0.193	& 0.078
	& \bred{0.324}	& \black{0.085}	& \black{0.037} \\
	
	
	
	
	
	
	{zebra $\rightarrow$ horse}
	& ?	& ?	& ?
	& ?	& ?	& ?
	%& 0.282	& 0.216	& 0.104
	& \bred{0.292}	& \black{0.126}	& \bred{0.050} \\
	
	
	
	
	{tree $\rightarrow$ palm tree}
	& ?	& ?	& ?
	& ?  & ?	& ?
	%& \bred{0.314}  & 0.129	& 0.046 
	& \bred{0.314}	& \black{0.085}	& \black{0.036} \\
	
	{dog $\rightarrow$ dog w/ glasses}
	& ?	& ?	& ?
	& ?	& ?	& ? 
	%& \black{0.322}	& 0.050	& \black{0.015} 
	& \bred{0.312}	& \black{0.026}	& \bred{0.016} \\
	
	\hline
	%\bottomrule 
\end{tabular}
%}
}
%
\label{tab:ablation}
\end{table*}
%
\fi
\iffalse
\begin{figure*}
\centering  
\subfigure[Subfigure a]{\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_1_2.pdf}}
\subfigure[Subfigure b]{\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_2_2.pdf}}
\subfigure[Subfigure c]{\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_3_2.pdf}}
%\subfigure[Subfigure c]{\includegraphics[width=0.45\linewidth]{example-image-a}}
\caption{Subfigures}
\end{figure*}
\fi


\subsection{Quantitative Results}
To compare the proposed method with state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}, we present quantitative results in \cref{tab:cmp_baselines}.
The table shows our method always achieves the best performance in background distance and mostly exceeds the previous methods in terms of structure distance.  
Regarding the CLIP similarity, the proposed method shows the highest performance on the dog $\rightarrow$ cat task, while it attains the second-highest performance on the other tasks.
Note that the CLIP similarity does not reflect the fidelity to source images and, according to our experience, it is not sufficiently discriminative to evaluate image-to-image translation performance.
%We emphasize that it is important to consider a comprehensive comparison through multiple metrics. 
%We empirically observe that the slight differences in CLIP similarity do not lead to perceptible qualitative results. 
%despite achieving the best or the second-best performance for all cases,  
%the marginal difference imperceptable since the score depends largely on the generated prompts given by BLIP~\cite{li2022blip}.
%outperforms the previous algorithms in terms of BD and SD 
In addition, \cref{tab:addon_ptp}, \cref{tab:addon_pnp}, and \cref{tab:addon_p2p} show that PIC is effective to enhance the performance of existing methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}.  





\subsection{Qualitative Results}
We visualize qualitative results generated by the proposed method and state-of-the-art frameworks~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero} in \cref{fig:comparisons}. 
The figure demonstrates that the proposed method effectively maintains the background or structure of the source image while selectively editing the region of interest. 
On the other hand, existing algorithms often fail to preserve the structure or background.
\cref{fig:addon} demonstrates that the proposed method is effective to improve the previous methods when integrated into them.

\subsection{Comparison of Inference Time}
To evaluate the realistic speed of each algorithm, we measure the wall-clock time using a single image on a NVIDIA A6000 GPU. %with a single image. 
As shown in \cref{tab:inference_time}, PIC is the most efficient even with its outstanding performance in the quality of translated images.

\begin{table}[t!]
	\centering
	\caption{
		Wall-clock inference time of the proposed method compared to existing state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}.%Inference Time (s)
	}
	%\vspace{-0.1in}
	%\vspace{0.1in}
	\setlength\tabcolsep{10pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\hspace{-2mm}
			\begin{tabular}{l c | c | c | c}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				%\hline
				\multirow{1}{*}{} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{1}{c|}{PtP}
				& \multicolumn{1}{c|}{PnP}
				& \multicolumn{1}{c|}{P2P} 
				& \multicolumn{1}{c}{PIC (Ours)} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\\ 
				\cline{1-5}
				%\cline{1-16}
				
				{Inference Time (s)}
				% & ? & ? & ?
				& 31.2 %& \bred{0.076} & 0.038 
				& \bred{24.4} % & 0.100 & \bred{0.032} 
				& 52.2 %& 0.127% & 0.099
				& \black{18.1} \\ %& \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:inference_time}
\end{table}


%%
%%
%%

\subsection{Ablation Study}
\begin{table*}[t!]
	\centering
	\caption{
		Contribution of the noise correction and the prompt interpolation tested on LAION-5B dataset~\cite{schuhmann2022laion}.
		`DDIM w/ PI' simply synthesizes target images by replacing $\epth(\bxtgt_t, t, \bytgt)$ with $\epth(\bxtgt_t, t, \by_t)$ during the reverse DDIM process in Eq. (3) of the main paper. %without using the noise correction term.
		For the noise correction term in Eq. (6), `DDIM w/ NC' substitutes $\epth(\bxtgt_t, t, \bytgt)$ for $\epth(\bxtgt_t, t, \by_t)$  without the consideration of the proposed prompt interpolation.
		%the interpolated embedding
		%Ablation study results to compare the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt}, Plug-and-Play~\cite{tumanyan2023plug}, and Pix2Pix-Zero~\cite{parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
		%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
		%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
		%
		% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
		%and the lower value does not imply that the algorithm achieves good performance.
		%Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
	}
	%\vspace{0.1in}
	%\vspace{-0.1in}
	\setlength\tabcolsep{2pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\hspace{-3mm}
			\begin{tabular}{l | ccc | ccc | ccc | ccc}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{3}{c|}{DDIM}
				& \multicolumn{3}{c|}{DDIM w/ PI}
				& \multicolumn{3}{c|}{DDIM w/ NC} 
				& \multicolumn{3}{c}{PIC (Ours)} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13}
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				%& CS ($\uparrow$)
				%& BD ($\downarrow$)
				%& SD ($\downarrow$)
				
				\\ 
				\cline{1-13}
				%\cline{1-16}
				
				{dog $\rightarrow$ cat}
				% & ? & ? & ?
				& \bred{0.289} & 0.158 & 0.086 
				& \bred{0.289} & 0.130 & 0.070
				& \black{0.293} & \bred{0.054} & \bred{0.038}
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				% & ? & ? & ?
				& 0.283 & 0.185 & 0.089
				& \bred{0.285} & 0.150 & 0.070
				& \black{0.288} & \bred{0.068} & \bred{0.041}
				& \black{0.288} & \black{0.057} & \black{0.033} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				% & ? & ? & ?
				& 0.325	& 0.287	& 0.123
				& \bred{0.330}	& 0.214	& 0.097
				& \black{0.333}	& \bred{0.113}	& \bred{0.050}
				& 0.324	& \black{0.085}	& \black{0.037} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				% & ? & ? & ?
				& \black{0.294}	& 0.295	& 0.104
				& \black{0.294}	& 0.254	& 0.097
				& \black{0.294}	& \bred{0.139}	& \bred{0.055}
				& \bred{0.292}	& \black{0.126}	& \black{0.050} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& 0.304	& 0.234	& 0.088
				& 0.306 & \bred{0.222}	& 0.084
				& \bred{0.312} & \black{0.085}	& \bred{0.056}
				& \black{0.314}	& \black{0.085}	& \black{0.036} \\
				% & \black{0.293} & \black{0.045} & \black{0.031}\\
				
				{dog $\rightarrow$ dog w/ glasses}
				& \black{0.318}	& 0.134	& 0.072
				& 0.310	& 0.132	& 0.065 
				& \bred{0.317}	& \bred{0.029}	& \bred{0.021}
				& 0.312	& \black{0.026}	& \black{0.016} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				
				\hline
				{Average}
				& 0.302	& 0.215	& 0.094
				& 0.302	& 0.184	& 0.080 
				& \black{0.306}	& \bred{0.081}	& \bred{0.043} 
				& \bred{0.304}	& \black{0.071}	& \black{0.034} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:ablation}
\end{table*}

\subsubsection{Prompt interpolation}
We conduct an ablation study to analyze the effect of each contribution tested on multiple text-driven image-to-image translation tasks.  
% As presented in Table~\cref{tab:ablation} and Figure~\ref{fig:ablation}, DDIM w/ PI is more effective than the standard DDIM~\cite{songdenoising}-based image editing, referred to as DDIM, where DDIM w/ PI replaces $\epth(\bxtgt_t, t, \bytgt)$ with $\epth(\bxtgt_t, t, \by_t)$ during the standard DDIM reverse process.
As presented in \cref{tab:ablation}, DDIM w/ PI is more effective than the standard DDIM~\cite{songdenoising}-based image editing, referred to as DDIM, where DDIM w/ PI replaces denoising network $\epth(\bxtgt_t, t, \bytgt)$ with $\epth(\bxtgt_t, t, \by_t)$ during the standard DDIM reverse process.
Moreover, when comparing DDIM with DDIM w/ NC, the proposed noise correction term is particularly helpful in preserving the background or structure of the source images. 
In case of DDIM w/ NC, we substitute $\epth(\bxtgt_t, t, \bytgt)$ for $\epth(\bxtgt_t, t, \by_t)$ to compute the noise correction term without using the proposed prompt interpolation $\by_t$.
Finally, our full model, which incorporates the noise correction term with the proposed text interpolation, achieves the best performance in text-conditional image editing tasks.


\vspace{-1em}
\subsubsection{Effect of $\gamma$}
%
We study the effect of $\gamma$ defined in  Eq.~\eqref{eq:new_noise_prediction2} to discuss the trade-off between fidelity to the target prompt and structure preservation, where $\gamma$ plays a crucial role in our image-to-image translation process. 
For the experiment, we use five different values of $\gamma$, $\{0.1, 0.2, 0.3, 0.4, 0.5 \}$ for PIC. 
As visualized in~\cref{fig:gamma}, out results are fairly consistent to the value of $\gamma$.
However, we observe that a lower value of $\gamma$ tends to preserve the structure or background with lower fidelity while a higher value of $\gamma$ enhances fidelity at the expense of structure deformation.
Note that our method reinstates the source images at $\gamma = 0.0$ and we use $\gamma = 0.2$ throughout all experiments.
%Note that when $\gamma$ is set to $0$, our method generates the source images for the text-driven image editing tasks. 
%
%Also, we empirically observe that a lower value of $\gamma$ preserves the structure or background with lower fidelity, while a higher value of $\gamma$ enhances fidelity at the expense of structure preservation. 
%$\gamma$ exhibits a trade-off between fidelity to the target prompt and structure preservation. 
%a lower value of $\gamma$ preserves the structure or background with lower fidelity, while a higher value of $\gamma$ enhances fidelity at the expense of structure preservation. 
%\cref{fig:gamma} displays translated images using various values of $\gamma$, where the optimal image quality is typically observed at $\gamma = 0.2$.%TODO: Add Figure + Explanation%

\begin{figure*}[t!]
	\centering
	%\vspace{-5pt}
	%\vspace{0.2cm}
	\includegraphics[width=\linewidth]{../figures/ICCV_Ablation_2row.pdf}
	%\vspace{-5pt}
	\caption{Qualitative results of the proposed method by varying $\gamma$ on data sampled from the LAION-5B dataset~\cite{schuhmann2022laion} relying on the pretrained Stable Diffusion~\cite{rombach2022high}. 
	%LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
	%Comparisons between various values of $\gamma$ in our proposed method. Optimal image quality usually observed at $\gamma=0.2$.
	}
	%Qualitative results of Pix2Pix on the Cityscapes dataset.
	% ``Output" denotes the ground-truth and ``Original" represents the uncompressed generator.}
%\vspace{0.3cm}
\label{fig:gamma}
\end{figure*}

==> sec/Experiment_copy.tex <==
% !TEX root = ./../main.tex
\section{Experiments}
\label{sec:experiments}
We evaluate the performance of our approach, PIC, in comparison with the state-of-the-art training-free diffusion-based image-to-image translation methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}. 
We denote the algorithms integrating PIC by `[Algorithm name] + PIC'.


%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative comparisons of PIC with Prompt-to-Prompt~\cite{hertz2023prompt}, Plug-and-Play~\cite{tumanyan2023plug}, and Pix2Pix-Zero~\cite{parmar2023zero} on images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high} backbone. 
		Black and red bold-faced numbers denote the best and second-best performances within each row for each metric. 
	}
	\setlength\tabcolsep{2pt} 
	%\hspace{-3mm}
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l | ccc | ccc | ccc | ccc}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{3}{c|}{PtP}
				& \multicolumn{3}{c|}{PnP}
				& \multicolumn{3}{c|}{P2P} 
				& \multicolumn{3}{c}{PIC (Ours)} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13}
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				%& CS ($\uparrow$)
				%& BD ($\downarrow$)
				%& SD ($\downarrow$)
				
				\\ 
				\cline{1-13}
				%\cline{1-16}
				
				{dog $\rightarrow$ cat}
				& \bred{0.290} & \bred{0.076} & 0.038 
				& \black{0.293} & 0.100 & \bred{0.032} 
				& 0.281 & 0.127 & 0.099
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				% & ? & ? & ?
				& \bred{0.288} & \bred{0.095} & \bred{0.042}
				& \black{0.291} & 0.099 & \black{0.033}
				& 0.282 & 0.100 & 0.054
				& \bred{0.288} & \black{0.057} & \black{0.033} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				% & ? & ? & ?
				& 0.320	& \bred{0.133}	& \bred{0.042}
				& \black{0.333}	& 0.158	& \bred{0.042}
				& 0.323	& 0.193	& 0.078
				& \bred{0.324}	& \black{0.085}	& \black{0.037} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				% & ? & ? & ?
				& 0.291	& 0.183	& 0.051
				& \black{0.299}	& \bred{0.152}	& \black{0.043}
				& 0.282	& 0.216	& 0.104
				& \bred{0.292}	& \black{0.126}	& \bred{0.050} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& \black{0.315}	& 0.147	& 0.045
				& \bred{0.314}  & \bred{0.122}	& \bred{0.039}
				& \bred{0.314}  & 0.129	& 0.046 
				& \bred{0.314}	& \black{0.085}	& \black{0.036} \\
				% & \black{0.293} & \black{0.045} & \black{0.031}\\
				
				{dog $\rightarrow$ dog w/glasses}
				& 0.310	& \bred{0.041}	& 0.020
				& 0.302	& 0.087	& 0.025 
				& \black{0.322}	& 0.050	& \black{0.015} 
				& \bred{0.312}	& \black{0.026}	& \bred{0.016} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				
				\hline
				{Average}
				& 0.302	& \bred{0.113}	& 0.040
				& \black{0.305}	& 0.120	& \bred{0.036} 
				& 0.301	& 0.136	& 0.066 
				& \bred{0.304}	& \black{0.071}	& \black{0.034} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	% 
	\label{tab:cmp_baselines} 
\end{table} %TODO: Reshape this table
%



\iffalse
%
\begin{table*}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt}, Plug-and-Play~\cite{tumanyan2023plug}, and Pix2Pix-Zero~\cite{parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
		%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
		%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
		%
		% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
		%and the lower value does not imply that the algorithm achieves good performance.
		Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
	}
	%\vspace{0.1in}
	\setlength\tabcolsep{3pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l ccc | ccc | ccc | ccc | ccc}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				\hline
				\multirow{2}{*}{Task} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{3}{c|}{DDIM}
				& \multicolumn{3}{c|}{PtP}
				& \multicolumn{3}{c|}{PnP} 
				& \multicolumn{3}{c|}{P2P}
				& \multicolumn{3}{c}{Ours} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline {14-16}
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-16}
				%\cline{1-16}
				
				{dog $\rightarrow$ cat}
				% & ? & ? & ?
				& 0.289 & 0.165 & 0.086
				& \bred{0.290} & \bred{0.076} & 0.038 
				& \black{0.293} & 0.100 & \bred{0.032} 
				& 0.281 & 0.127 & 0.099
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				% & ? & ? & ?
				& 0.282 & 0.188 & 0.089
				& \bred{0.288} & \bred{0.095} & \bred{0.042}
				& \black{0.291} & 0.099 & \black{0.033}
				& 0.282 & 0.100 & 0.054
				& \bred{0.288} & \black{0.057} & \black{0.033} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				% & ? & ? & ?
				& \bred{0.325}	& 0.299	& 0.123
				& 0.320	& \bred{0.133}	& \bred{0.042}
				& \black{0.333}	& 0.158	& \bred{0.042}
				& 0.323	& 0.193	& 0.078
				& 0.324	& \black{0.085}	& \black{0.037} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				% & ? & ? & ?
				& \bred{0.294}	& 0.301	& 0.104
				& 0.291	& 0.183	& 0.051
				& \black{0.299}	& \bred{0.152}	& \black{0.043}
				& 0.282	& 0.216	& 0.104
				& 0.292	& \black{0.126}	& \bred{0.050} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& 0.304	& 0.236	& 0.088
				& \black{0.315}	& 0.147	& 0.045
				& \bred{0.314}  & \bred{0.122}	& \bred{0.039}
				& \bred{0.314}  & 0.129	& 0.046 
				& \bred{0.314}	& \black{0.085}	& \black{0.036} \\
				% & \black{0.293} & \black{0.045} & \black{0.031}\\
				
				{dog $\rightarrow$ dog w/ glasses}
				& \bred{0.318}	& 0.137	& 0.072
				& 0.310	& \bred{0.041}	& 0.020
				& 0.302	& 0.087	& 0.025 
				& \black{0.322}	& 0.050	& \black{0.015} 
				& 0.312	& \black{0.026}	& \bred{0.016} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				
				\hline
				{Average}
				& 0.302	& 0.221	& 0.093
				& 0.302	& \bred{0.113}	& 0.040
				& \black{0.305}	& 0.120	& \bred{0.036} 
				& 0.301	& 0.136	& 0.066 
				& \bred{0.304}	& \black{0.071}	& \black{0.034} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:cmp_baselines}
\end{table*}
%
\fi
\iffalse
%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative results to compare the proposed method with DDIM on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pre-trained Stable Diffusion~\cite{rombach2022high} when the proposed method is integrated with Prompt-to-Prompt.
		%Plug-and-Play~\citep{tumanyan2023plug}, and Pix2Pix-Zero~\citep{parmar2023zero} on real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} using the pre-trained Stable Diffusion~\citep{rombach2022high}.  
		%Note that 
		The results of Prompt-to-Prompt are retrieved from \cref{tab:cmp_baselines}.
		Black bold-faced numbers represent better performance for each metric in each row. 
	}
	%\vspace{0.1in}
	\setlength\tabcolsep{3pt} 
	\scalebox{0.80}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l ccc | ccc }
				%\toprule 
				\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{DDIM}
				& \multicolumn{3}{c}{Ours}\\
				
				\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				& 0.289 & 0.165 & 0.086
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& 0.281 & 0.127 & 0.099
				%& \black{0.293} & \black{0.046} & \black{0.031} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				& 0.282 & 0.188 & 0.089
				& \black{0.288} & \black{0.057} & \black{0.033} \\
				%& 0.282 & 0.100 & 0.054
				%& \red{0.288} & \black{0.060} & \red{0.034} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				& \black{0.325}	& 0.299	& 0.123
				& 0.324	& \black{0.085}	& \black{0.037} \\
				%& 0.323	& 0.193	& 0.078
				%& \red{0.324}	& \black{0.133}	& \black{0.036} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				& \black{0.294}	& 0.301	& 0.104
				& 0.292	& \black{0.126}	& \black{0.050} \\
				%& 0.282	& 0.216	& 0.104
				%& \red{0.293}	& \black{0.086}	& \red{0.051} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& 0.304	& 0.236	& 0.088
				& \black{0.314}	& \black{0.085}	& \black{0.036} \\
				%& 0.314	& -	& 0.046 
				%& 0.314	& -	& 0.043 \\
				
				{dog $\rightarrow$ dog w/ glasses}
				& \black{0.318}	& 0.137	& 0.072
				& 0.312	& \black{0.026}	& \black{0.016} \\
				%& \black{0.322}	& 0.050	& \black{0.015} 
				%& \red{0.316}	& \black{0.037}	& 0.022 \\
				
				\hline
				{Average}
				& 0.302	& 0.221	& 0.093
				& \black{0.304}	& \black{0.071}	& \black{0.034} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	%
	\label{tab:addon_ptp}
\end{table}
%
\fi
%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative comparisons of the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt} on images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
		Out technique is integrated into Prompt-to-Prompt and the results of Prompt-to-Prompt are obtained from \cref{tab:cmp_baselines}.
		Black bold-faced numbers represent better performance on each metric between two approaches. 
	}
	\setlength\tabcolsep{8pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l | ccc | ccc }
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{PtP}
				& \multicolumn{3}{c}{PtP + PIC (Ours)}\\
				
				%\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				& \black{0.290} & 0.076 & 0.038 
				& 0.283 & \black{0.051} & \black{0.021}  \\
				%& 0.281 & 0.127 & 0.099
				%& \black{0.293} & \black{0.046} & \black{0.031} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				& 0.288 & 0.095 & 0.042 
				& \black{0.291} & \black{0.052} & \black{0.027} \\
				%& 0.282 & 0.100 & 0.054
				%& \red{0.288} & \black{0.060} & \red{0.034} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				& \black{0.320}	& 0.133	& 0.042
				& 0.292	& \black{0.071}	& \black{0.018} \\
				%& 0.323	& 0.193	& 0.078
				%& \red{0.324}	& \black{0.133}	& \black{0.036} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				& \black{0.291}	& 0.183	& 0.051
				& 0.290	& \black{0.131}	& \black{0.034} \\
				%& 0.282	& 0.216	& 0.104
				%& \red{0.293}	& \black{0.086}	& \red{0.051} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& \black{0.315}	& 0.147	& 0.045
				& 0.301	& \black{0.070}	& \black{0.026} \\
				%& 0.314	& -	& 0.046 
				%& 0.314	& -	& 0.043 \\
				
				{dog $\rightarrow$ dog w/glasses}
				& \black{0.310}	& 0.041	& 0.020
				& 0.301	& \black{0.038}	& \black{0.011} \\
				%& \black{0.322}	& 0.050	& \black{0.015} 
				%& \red{0.316}	& \black{0.037}	& 0.022 \\
				
				\hline
				{Average}
				& \black{0.302}	& 0.113	& 0.040
				& 0.295	& \black{0.069}	& \black{0.023} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	%
	\label{tab:addon_ptp}
\end{table}

\subsection{Implementation Details}
We implement the proposed method using the publicly available code of Pix2Pix-Zero (P2P)\footnote{\url{https://github.com/pix2pixzero/pix2pix-zero}}.
We integrate PIC into the existing techniques---Prompt-to-Prompt (PtP)\footnote{\url{https://github.com/google/prompt-to-prompt}}, Plug-and-Play (PnP)\footnote{\url{https://github.com/MichalGeyer/plug-and-play}} and Pix2Pix-Zero (P2P)---using their official codes.
% Also, we integrate our algorithm into the existing techniques---Prompt-to-Prompt (PtP)\footnote{\url{https://github.com/google/prompt-to-prompt}} and Plug-and-Play (PnP)\footnote{\url{https://github.com/MichalGeyer/plug-and-play}}---using their official codes.
To accelerate the text-driven image-to-image translation process, the inference time steps for the forward and reverse processes are set to $50$. For all experiments, \bhr{Stable Diffusion v1.4 is employed as the backbone model.}
During the forward process, we adopt Bootstrapping Language-Image Pretraining (BLIP)~\cite{li2022blip} to generate a source prompt for conditioning the denoising network.   
The target prompt is given by replacing the specific words in the source prompt with the alternatives defined by an assigned task as mentioned in Section~\ref{subsec:text_embedding_interpolation}.
We use the same source and target prompts of all algorithms for the fair comparisons during both the forward and reverse processes. 
Additionally, we adopt classifier-free guidance~\cite{ho2021classifier} following~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}. 

In our implementation, $\tau$ and $\gamma$ are set to $25$ and $1.0$, respectively, for all experiments. 
Also, we set $\beta$ to $0.3$ for word replacement tasks (\eg `dog $\rightarrow$ cat' and `horse $\rightarrow$ zebra') while it is set to $0.8$ for adding phrases tasks (\eg `tree $\rightarrow$ palm tree' and `dog $\rightarrow$ dog with glasses').


%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative comparisons of the proposed method with Plug-and-Play~\cite{tumanyan2023plug} on images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
		Out technique is integrated into Plug-and-Play and the results of Plug-and-Play are obtained from~\cref{tab:cmp_baselines}.
	}
	%\vspace{-0.1in}
	%\vspace{0.1in}
	\setlength\tabcolsep{8pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l | ccc | ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{PnP}
				& \multicolumn{3}{c}{PnP + PIC (Ours)}\\
				
				%\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				%& \red{0.290} & \red{0.076} & 0.038 
				& \black{0.293} & 0.100 & 0.032  
				& 0.282 & \black{0.092} & \black{0.027} \\
				%& \black{0.293} & \black{0.046} & \black{0.031} \\			
						
				
				{cat $\rightarrow$ dog}
				%& \red{0.288} & \red{0.095} & 0.042 
				& \black{0.291} & 0.099 & 0.033 
				& 0.288 & \black{0.083} & \black{0.028} \\
				%& \red{0.288} & \black{0.060} & \red{0.034} \\
				
							
				{horse $\rightarrow$ zebra}
				%& 0.320	& \black{0.133}	& \red{0.042}
				& \black{0.333}	& 0.158	& 0.042 
				& 0.317	& \black{0.121}	& \black{0.035} \\
				%& \red{0.324}	& \black{0.133}	& \black{0.036} \\
				
							
				{zebra $\rightarrow$ horse}
				%& 0.291	& 0.183	& 0.051
				& \black{0.299}	& 0.152	& 0.043 
				& 0.285	& \black{0.135}	& \black{0.037} \\
				%& \red{0.293}	& \black{0.086}	& \red{0.051} \\
				
						
				{tree $\rightarrow$ palm tree}
				%& 0.315	& -	& 0.045
				& \black{0.314}	& 0.122	& 0.039 
				& 0.295	& \black{0.070} & \black{0.024}  \\
				%& 0.314	& -	& 0.043 \\
				
				{dog $\rightarrow$ dog w/glasses}
				%& 0.310	& \red{0.041}	& \red{0.020}
				& \black{0.302}	& 0.087	& 0.025 
				& 0.300	& \black{0.085}	& \black{0.024} \\
				%& \red{0.316}	& \black{0.037}	& 0.022 \\
				
				\hline
				{Average}
				& \black{0.305}	& 0.120	& 0.036 
				& 0.295	& \black{0.098}	& \black{0.029} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			
			
			%}
	}
	%
	\label{tab:addon_pnp}
\end{table}
%


%
\begin{table}[t!]
	\centering
	\caption{
		Quantitative comparisons of the proposed method with Pix2Pix-Zero~\cite{parmar2023zero} on images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
		Out technique is integrated into Pix2Pix-Zero and the results of Pix2Pix-Zero are obtained from~\cref{tab:cmp_baselines}.
	}
	%\vspace{0.1in}
	%\vspace{-0.1in}
	\setlength\tabcolsep{8pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l | ccc | ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				& \multicolumn{3}{c|}{P2P}
				& \multicolumn{3}{c}{P2P + PIC (Ours)}\\
				
				%\cline{2-4} \cline{5-7} %\cline{8-10} \cline{11-13}
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				\\ 
				\cline{1-7}
				
				{dog $\rightarrow$ cat}
				%& \red{0.290} & \red{0.076} & 0.038 
				%& \black{0.293} & 0.100 & \red{0.032}  \\
				& 0.281 & 0.127 & 0.099
				& \black{0.282} & \black{0.051} & \black{0.017} \\
				
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				%& \red{0.288} & \red{0.095} & 0.042 
				%& \black{0.291} & 0.099 & \black{0.033} \\
				& 0.282 & 0.100 & 0.054
				& \black{0.285} & \black{0.056} & \black{0.016} \\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				%& 0.320	& \black{0.133}	& \red{0.042}
				%& \black{0.333}	& 0.158	& \red{0.042} \\
				& \black{0.323}	& 0.193	& 0.078
				& 0.309	& \black{0.070}	& \black{0.016} \\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				%& 0.291	& 0.183	& 0.051
				%& \black{0.299}	& \red{0.152}	& \black{0.043} \\
				& \black{0.282}	& 0.216	& 0.104
				& 0.279	& \black{0.117}	& \black{0.017} \\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				%& 0.315	& -	& 0.045
				%& ?	& -	& ? \\
				& 0.314	& 0.129	& 0.046 
				& \black{0.298}	& \black{0.047}	& \black{0.014} \\
				
				{dog $\rightarrow$ dog w/glasses}
				%& 0.310	& \red{0.041}	& \red{0.020}
				%& 0.302	& 0.087	& 0.025 \\
				& \black{0.322}	& \black{0.050}	& 0.015 
				& 0.302	& 0.053	& \black{0.011} \\
				
				
				
				\hline
				{Average}
				%& 0.310	& \red{0.041}	& \red{0.020}
				%& 0.302	& 0.087	& 0.025 \\
				& \black{0.301}	& 0.136	& 0.066 
				& 0.293	& \black{0.066}	& \black{0.015} \\
				
				
				\hline
				%\bottomrule 
			\end{tabular}
			%}
	}
	%
	\label{tab:addon_p2p}
\end{table}
%
\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{./figures/CVPR_Comparison.pdf}
	%\vspace{-5pt}
	\caption{Qualitative comparisons between PIC and state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero} on images from LAION-5B~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
		PIC generates target images with higher-fidelity than others. 
	}
\label{fig:comparisons}
\end{figure}
%
\begin{figure}
\begin{subfigure}{\linewidth}
	\centering
	\includegraphics[width=1.0\linewidth]{./figures/CVPR_Addon_1_2.pdf}
	%\caption{Prompt-to-Prompt~\cite{hertz2023prompt}}
	%\label{fig:first}
\end{subfigure}
\begin{subfigure}{\linewidth}
	\centering
	\includegraphics[width=1.0\linewidth]{./figures/CVPR_Addon_2_2.pdf}
	%\caption{Plug-and-Play~\cite{tumanyan2023plug}}
	%\label{fig:second}
\end{subfigure}
\begin{subfigure}{\linewidth}
	\centering
	\includegraphics[width=1.0\linewidth]{./figures/CVPR_Addon_3_2.pdf}
	%\caption{Pix2Pix-Zero~\cite{parmar2023zero}}
	%\label{fig:third}
\end{subfigure}
%\vspace{3pt}
\caption{Qualitative results of existing state-of-the-art methods and their combinations with PIC based on the pretrained Stable Diffusion~\cite{rombach2022high}: (top) Prompt-to-Prompt~\cite{hertz2023prompt}, (middle) Plug-and-Play~\cite{tumanyan2023plug}, and (bottom) Pix2Pix-Zero~\cite{parmar2023zero}.
The examples are sampled from LAION-5B~\cite{schuhmann2022laion}.
	%The proposed method is effective to preserve the structure or background when combined with the previous frameworks.
}
%Prompt-to-Prompt~\cite{}, Plug-and-Play~\cite{}, Pix2Pix-Zero~\cite{}, and }
\label{fig:addon}
\end{figure}


\subsection{Evaluation Metrics}
For quantitative evaluations, we measure CLIP Similarity (CS)~\cite{hessel2021clipscore}, Background Distance (BD), and Structure Distance (SD)~\cite{tumanyan2022splicing} following Pix2Pix-Zero~\cite{parmar2023zero}. 
To obtain the scores of these metrics, we choose $250$ images deemed most relevant to a given task based on the CLIP Similarity, which quantifies how well the translated images are aligned with the target prompts.
%To this end, we measure the cosine similarity between the CLIP embeddings of target images and target prompts. 
On the other hand, the background distance calculates the Learned Perceptual Image Patch Similarity (LPIPS) score~\cite{zhang2018unreasonable} between the background regions of the source and translated images.
To identify background regions, we employ the prediction of the pretrained object detector~\cite{ren2024grounded}.
The structure distance~\cite{tumanyan2022splicing} is employed to evaluate the structural difference between the source and translated images. 
\bhb{It computes the Frobenius norm between the self-attention maps from the DINO-ViT network~\cite{caron2021emerging} given the source and translated images as inputs.}
%using the source and translated results as inputs, respectively.
%Lower structure distance values imply that the translation images more effectively maintains the structure in the source images.


%\paragraph{CLIP Similarity (CS)}
%CLIP similarity~\cite{hessel2021clipscore} quantifies how well the translated images are aligned with the target prompts.
%To this end, we measure the cosine similarity between two CLIP embeddings of the target images and target prompts. 
%given by the pretrained CLIP image encoder and text encoder, respectively.  
%The higher CLIP similarity implies that 





%\subsubsection{Background Distance (BD)}
%\paragraph{Background Distance (BD)} 
%Background distance calculates the Learned Perceptual Image Patch Similarity (LPIPS) score~\cite{zhang2018unreasonable} between the background regions of the source and target images.
%In order to estimate the background region, we employ the prediction of the pretreined object detector~\cite{zhou2022detecting}. 
%Lower values of the background distance suggest that the background regions of the source images are better preserved in the translated results. 





%\subsubsection{Structure Distance (SD)}
%\paragraph{Structure Distance (SD)}
%Structure distance~\cite{tumanyan2022splicing} is employed to evaluate the structural difference between the source and translated images. 
%It computes the Frobenius norm between two self-attention maps given by the DINO-ViT network output~\cite{caron2021emerging} using the source and translated results as inputs, %respectively. 
%Lower structure distance values imply that the translation images more effectively maintains the structure in the source images.








\iffalse
%
\begin{figure*}[t!]
\centering
%\vspace{-5pt}
%\vspace{0.2cm}
\includegraphics[width=0.90\linewidth]{../figures/CVPR_Addon.pdf}
%\vspace{-5pt}
\caption{\ms{TODO TODO TODO}}
%Qualitative results of Pix2Pix on the Cityscapes dataset.
% ``Output" denotes the ground-truth and ``Original" represents the uncompressed generator.}
%\vspace{0.3cm}
\label{fig:comparisons}
\end{figure*}
%
\fi




\iffalse
%
\begin{table*}[t!]
\centering
\caption{
Ablation study results on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
%
% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
%and the lower value does not imply that the algorithm achieves good performance.
%Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
}
%\vspace{0.1in}
\setlength\tabcolsep{3pt} 
\scalebox{0.80}{
%\resizebox{\linewidth}{!}{
\begin{tabular}{l ccc ccc ccc}
	%\toprule 
	\hline
	\multirow{2}{*}{Task} 
	& \multicolumn{3}{c}{DDIM}
	& \multicolumn{3}{c}{Prompt Interpolation}
	%& \multicolumn{3}{c}{P2P} 
	& \multicolumn{3}{c}{Ours} \\
	
	\cline{2-4} \cline{5-7} \cline{8-10} %\cline{11-13}
	
	& CS ($\uparrow$)
	& BD ($\downarrow$)
	& SD ($\downarrow$)
	
	
	& CS ($\uparrow$)
	& BD ($\downarrow$)
	& SD ($\downarrow$)
	
	& CS ($\uparrow$)
	& BD ($\downarrow$)
	& SD ($\downarrow$)
	
	
	
	
	\\ 
	\cline{1-10}
	
	{dog $\rightarrow$ cat}
	& ? & ? & ? 
	& ? & ? & ? 
	%& 0.281 & 0.127 & 0.099
	& \black{0.293} & \black{0.045} & \black{0.031} \\
	
	
	
	
	
	
	
	{cat $\rightarrow$ dog}
	& ? & ? & ?
	& ? & ? & ?
	%& 0.282 & 0.100 & 0.054
	& \bred{0.288} & \black{0.057} & \black{0.033} \\
	
	
	
	
	
	{horse $\rightarrow$ zebra}
	& ?	& ?	& ?
	& ?	& ?	& ?
	%& 0.323	& 0.193	& 0.078
	& \bred{0.324}	& \black{0.085}	& \black{0.037} \\
	
	
	
	
	
	
	{zebra $\rightarrow$ horse}
	& ?	& ?	& ?
	& ?	& ?	& ?
	%& 0.282	& 0.216	& 0.104
	& \bred{0.292}	& \black{0.126}	& \bred{0.050} \\
	
	
	
	
	{tree $\rightarrow$ palm tree}
	& ?	& ?	& ?
	& ?  & ?	& ?
	%& \bred{0.314}  & 0.129	& 0.046 
	& \bred{0.314}	& \black{0.085}	& \black{0.036} \\
	
	{dog $\rightarrow$ dog w/ glasses}
	& ?	& ?	& ?
	& ?	& ?	& ? 
	%& \black{0.322}	& 0.050	& \black{0.015} 
	& \bred{0.312}	& \black{0.026}	& \bred{0.016} \\
	
	\hline
	%\bottomrule 
\end{tabular}
%}
}
%
\label{tab:ablation}
\end{table*}
%
\fi
\iffalse
\begin{figure*}
\centering  
\subfigure[Subfigure a]{\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_1_2.pdf}}
\subfigure[Subfigure b]{\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_2_2.pdf}}
\subfigure[Subfigure c]{\includegraphics[width=1.0\linewidth]{../figures/CVPR_Addon_3_2.pdf}}
%\subfigure[Subfigure c]{\includegraphics[width=0.45\linewidth]{example-image-a}}
\caption{Subfigures}
\end{figure*}
\fi


\subsection{Quantitative Results}
To compare the proposed method with state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}, we present quantitative results in \cref{tab:cmp_baselines}.
The table shows that our method consistently achieves the best performance in the background distance and mostly outperforms
the previous methods for the structure distance.  
In terms of the CLIP similarity, the proposed method shows the highest performance on the dog $\rightarrow$ cat task, while it ranks second on the rest of the tasks.
Note that, because the CLIP similarity only reflects the fidelity to the target prompt without considering the similarity to source images, it is not sufficiently discriminative to evaluate image-to-image translation performance by itself.
%We emphasize that it is important to consider a comprehensive comparison through multiple metrics. 
%We empirically observe that the slight differences in CLIP similarity do not lead to perceptible qualitative results. 
%despite achieving the best or the second-best performance for all cases,  
%the marginal difference imperceptable since the score depends largely on the generated prompts given by BLIP~\cite{li2022blip}.
%outperforms the previous algorithms in terms of BD and SD 
In addition, \cref{tab:addon_ptp,tab:addon_pnp,tab:addon_p2p} demonstrate that PIC is effective to improve the performance when incorporated into existing methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}.  







\subsection{Qualitative Results}
\cref{fig:comparisons} illustrates qualitative results generated by the proposed approach and other state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}. 
It presents that our method effectively preserves the background and structure of source images while selectively editing the region of interest. 
On the other hand, existing algorithms often fail to preserve the structure or background.
\cref{fig:addon} demonstrates that PIC is effective to improve the previous methods when integrated into them.







\subsection{Inference Time}
To evaluate the inference time of each algorithm, we measure the wall-clock time using a single image on an NVIDIA A6000 GPU. 
As shown in \cref{tab:inference_time}, PIC is the most efficient even with its outstanding performance.

\begin{table}[t!]
	\centering
	\caption{
		Inference time comparisons between PIC and other state-of-the-art methods~\cite{hertz2023prompt, tumanyan2023plug, parmar2023zero}.%Inference Time (s)
	}
	\setlength\tabcolsep{16pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{c | c | c | c | c}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				%\hline
				%& \multicolumn{3}{c}{DDIM}
				
				& PtP
				& PnP
				& P2P 
				& PIC (Ours) \\ 
				\hline
				
				Inference time (s)
				& 31.2 %& \bred{0.076} & 0.038 
				& \bred{24.4} % & 0.100 & \bred{0.032} 
				& 52.2 %& 0.127% & 0.099
				& \black{18.1} \\ %& \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
								
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:inference_time}
\end{table}


%%
%%
%%

\subsection{Ablation Study}
\begin{table*}[t!]
	\centering
	\caption{
		Contribution of the noise correction and the prompt interpolation tested on LAION-5B dataset~\cite{schuhmann2022laion}.
		DDIM+PI synthesizes target images by replacing $\epth(\bxtgt_t, t, \bytgt)$ with $\epth(\bxtgt_t, t, \by_t)$ in the reverse DDIM process. 
		The model with the noise correction, DDIM+NC, substitutes $\epth(\bxtgt_t, t, \bytgt)$ for $\epth(\bxtgt_t, t, \by_t)$  without the consideration of the prompt interpolation.
		%the interpolated embedding
		%Ablation study results to compare the proposed method with Prompt-to-Prompt~\cite{hertz2023prompt}, Plug-and-Play~\cite{tumanyan2023plug}, and Pix2Pix-Zero~\cite{parmar2023zero} on real images sampled from the LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}. 
		%and real images sampled from the LAION-5B dataset~\citep{schuhmann2022laion} for various tasks.
		%  text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from LAION 5B dataset~\citep{schuhmann2022laion} for various tasks. 
		%
		% For the the drawing $\rightarrow$ oil painting task, we do not report the BD score since the background can not be clearly defined.
		%and the lower value does not imply that the algorithm achieves good performance.
		%Black and red bold-faced numbers represent the best and second-best performances for each metric in each row. 
	}
	%\vspace{0.1in}
	%\vspace{-0.1in}
	\setlength\tabcolsep{2pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{l | ccc | ccc | ccc | ccc}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				%\hline
				\multirow{2}{*}{Task} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{3}{c|}{DDIM}
				& \multicolumn{3}{c|}{DDIM+PI}
				& \multicolumn{3}{c|}{DDIM+NC} 
				& \multicolumn{3}{c}{PIC (Ours)} \\ 
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13}
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				
				& CS ($\uparrow$)
				& BD ($\downarrow$)
				& SD ($\downarrow$)
				
				%& CS ($\uparrow$)
				%& BD ($\downarrow$)
				%& SD ($\downarrow$)
				
				\\ 
				\cline{1-13}
				%\cline{1-16}
				
				{dog $\rightarrow$ cat}
				% & ? & ? & ?
				& \bred{0.289} & 0.158 & 0.086 
				& \bred{0.289} & 0.130 & 0.070
				& \black{0.293} & \bred{0.054} & \bred{0.038}
				& \black{0.293} & \black{0.045} & \black{0.031} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{cat $\rightarrow$ dog}
				% & ? & ? & ?
				& 0.283 & 0.185 & 0.089
				& \bred{0.285} & 0.150 & 0.070
				& \black{0.288} & \bred{0.068} & \bred{0.041}
				& \black{0.288} & \black{0.057} & \black{0.033} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				{horse $\rightarrow$ zebra}
				% & ? & ? & ?
				& 0.325	& 0.287	& 0.123
				& \bred{0.330}	& 0.214	& 0.097
				& \black{0.333}	& \bred{0.113}	& \bred{0.050}
				& 0.324	& \black{0.085}	& \black{0.037} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				
				
				{zebra $\rightarrow$ horse}
				% & ? & ? & ?
				& \black{0.294}	& 0.295	& 0.104
				& \black{0.294}	& 0.254	& 0.097
				& \black{0.294}	& \bred{0.139}	& \bred{0.055}
				& \bred{0.292}	& \black{0.126}	& \black{0.050} \\
				%& \black{0.293} & \black{0.045} & \black{0.031}\\
				
				
				
				
				{tree $\rightarrow$ palm tree}
				& 0.304	& 0.234	& 0.088
				& 0.306 & \bred{0.222}	& 0.084
				& \bred{0.312} & \black{0.085}	& \bred{0.056}
				& \black{0.314}	& \black{0.085}	& \black{0.036} \\
				% & \black{0.293} & \black{0.045} & \black{0.031}\\
				
				{dog $\rightarrow$ dog w/glasses}
				& \black{0.318}	& 0.134	& 0.072
				& 0.310	& 0.132	& 0.065 
				& \bred{0.317}	& \bred{0.029}	& \bred{0.021}
				& 0.312	& \black{0.026}	& \black{0.016} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				
				\hline
				{Average}
				& 0.302	& 0.215	& 0.094
				& 0.302	& 0.184	& 0.080 
				& \black{0.306}	& \bred{0.081}	& \bred{0.043} 
				& \bred{0.304}	& \black{0.071}	& \black{0.034} \\
				%& \black{0.293} & \black{0.045} & \black{0.031} \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:ablation}
\end{table*}






\subsubsection{Prompt Interpolation}
To analyze the impact of each component in our algorithm, we compare PIC with its three variations---DDIM, DDIM+PI, and DDIM+NC.
DDIM denotes a na\"ive application of the original DDIM algorithm~\cite{song2021denoising} to image-to-image translation.
DDIM+PI replaces the denoising network $\epth(\bxtgt_t, t, \bytgt)$ in Eq.~\eqref{eq:naive_target} with $\epth(\bxtgt_t, t, \by_t)$ using interpolated prompts $\by_t$ while DDIM+NC substitutes $\epth(\bxtgt_t, t, \bytgt)$ for $\epth(\bxtgt_t, t, \by_t)$ in Eq.~\eqref{eq:new_noise_prediction2} to compute the noise correction term without the proposed prompt interpolation.
As presented in \cref{tab:ablation}, DDIM+PI improves performance by using prompt interpolation compared with the standard DDIM and DDIM+NC is particularly helpful in preserving the background or structure of the source images by integrating the noise correction term.
Our algorithm, PIC, incorporating both the noise correction term and the prompt interpolation, achieves the best performance in the text-conditional image editing task. The qualitative results are presented in Fig. 6 of the appendix. 

\iffalse
As presented in \cref{tab:ablation}, DDIM w/ PI is more effective than the standard DDIM~\cite{song2021denoising}-based image editing, referred to as DDIM, where DDIM w/ PI replaces denoising network $\epth(\bxtgt_t, t, \bytgt)$ with $\epth(\bxtgt_t, t, \by_t)$ during the standard DDIM reverse process.
Moreover, when comparing DDIM with DDIM w/ NC, the proposed noise correction term is particularly helpful in preserving the background or structure of the source images. 
In case of DDIM w/ NC, we substitute $\epth(\bxtgt_t, t, \bytgt)$ for $\epth(\bxtgt_t, t, \by_t)$ to compute the noise correction term without using the proposed prompt interpolation $\by_t$.
Finally, our full model, which incorporates the noise correction term with the proposed text interpolation, achieves the best performance in text-conditional image editing tasks.
\fi


\iffalse
We conduct an ablation study to analyze the impact of each component in our algorithm on multiple text-driven image-to-image translation tasks.  
As presented in \cref{tab:ablation}, DDIM w/ PI is more effective than the standard DDIM~\cite{song2021denoising}-based image editing, referred to as DDIM, where DDIM w/ PI replaces denoising network $\epth(\bxtgt_t, t, \bytgt)$ with $\epth(\bxtgt_t, t, \by_t)$ during the standard DDIM reverse process.
Moreover, when comparing DDIM with DDIM w/ NC, the proposed noise correction term is particularly helpful in preserving the background or structure of the source images. 
In case of DDIM w/ NC, we substitute $\epth(\bxtgt_t, t, \bytgt)$ for $\epth(\bxtgt_t, t, \by_t)$ to compute the noise correction term without using the proposed prompt interpolation $\by_t$.
Finally, our full model, which incorporates the noise correction term with the proposed text interpolation, achieves the best performance in text-conditional image editing tasks.
\fi






%\vspace{-1em}
\subsubsection{Effect of Hyperparameters}
%
We study the effect of hyperparameters $\gamma$, $\beta$ and $\tau$ introduced in our algorithm
%Eq.~\eqref{eq:new_noise_prediction2}
to discuss the trade-off between the fidelity to the target prompt and the structure preservation.

For the experiment related to $\gamma$, we explore five different values of $\gamma \in \{0.5, 1.0, 1.5, 2.0, 2.5 \}$ for PIC. \cref{fig:gamma} illustrates that our results are fairly consistent to the value of $\gamma$.
However, we observe that a low value of $\gamma$ tends to preserve the structure or background with relatively low fidelity, while a high value of $\gamma$ enhances fidelity at the expense of structure deformation. Note that we use $\gamma = 1.0$ throughout all experiments.

Next, we analyze the effect of $\tau$ and $\beta$ in Table~\ref{tab:hyperparameter}, which demonstrates that our method is robust to $(\beta, \tau)$. A high $\beta$ or low $\tau$ tends to increase fidelity to the target prompt, resulting in worse BD and SD scores. Conversely, a low $\beta$ or high $\tau$ enhance the preservation of background or structure in the source images, while decreasing the CS score.
Throughout our experiments, we set $\tau = 25$ and $\beta = 0.3$ for word-swap cases, while $\beta=0.8$ for adding phrases cases.

\iffalse
\subsection{Effect of adaptive interpolation in adding-phrase cases}
Our strategy for phrase-adding cases in Eq.~(10) simply matches the tokens between the source and target prompts, where the target tokens are used for the added phrase because it doesn't exist in the source prompt. Each token embedding is influenced by the preceding token embeddings. Therefore, we consider this as the adaptive interpolation.

Fig.~\ref{fig:simplelerp} presents a comparison between PIC and PIC with simple LERP. The latter fails to adequately preserve both the background and the structure of the object, whereas PIC maintains both effectively. So, we conclude that our token-matching interpolation significantly enhances the performance of our method.
\fi

\iffalse
\begin{table}[t!]
	\centering
	\caption{
		Results by varying $(\beta, \tau$) on the horse $\rightarrow$ zebra task.
	}
	%\vspace{0.1in}
	%\setlength\tabcolsep{1.7pt} 
	\scalebox{0.8}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{c| ccc ccc| c}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				\hline
				{($\beta$, $\tau$)} 
				%& \multicolumn{3}{c}{DDIM}
				& (0.1, 25) & (0.3, 25) & (0.5, 25) & (0.3, 15) & (0.3, 25) & (0.3, 35) &Avg.
				%& \multicolumn{1}{c}{std}
				\\ \hline
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				
				%\cline{1-16}
				
				{CS}
				& 0.322 & 0.324	& 0.329
				& 0.332 & 0.324 & 0.300
				& 0.322 $\pm$ 0.011 \\
				
				{BD}
				& 0.077 & 0.085	& 0.097
				& 0.183 & 0.085 & 0.035 
				& 0.094 $\pm$  0.049 \\
				
				{SD}
				& 0.033 & 0.037	& 0.041
				& 0.065 & 0.037 & 0.020 
				& 0.039 $\pm$ 0.015 \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:hyperparameter_1}
\end{table}

\begin{table}[t!]
	\centering
	\caption{
		Results by varying $(\beta, \tau$) on the dog $\rightarrow$ dog wearing glasses task.
	}
	%\vspace{0.1in}
	%\setlength\tabcolsep{1.7pt} 
	\scalebox{0.8}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{c| ccc ccc| c}
				%\begin{tabular}{l ccc ccc ccc ccc ccc}
				%\toprule 
				\hline
				{($\beta$, $\tau$)} 
				%& \multicolumn{3}{c}{DDIM}
				& (0.6, 25) & (0.8, 25) & (1.0, 25) & (0.8, 15) & (0.8, 25) & (0.8, 35) &Avg.
				%& \multicolumn{1}{c}{std}
				\\ \hline
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				
				%\cline{1-16}
				
				{CS}
				& 0.309 & 0.312	& 0.319
				& 0.317 & 0.312 & 0.307
				& 0.313 $\pm$ 0.005 \\
				
				{BD}
				& 0.025 & 0.026	& 0.035
				& 0.068 & 0.026 & 0.017 
				& 0.033 $\pm$  0.018 \\
				
				{SD}
				& 0.015 & 0.016	& 0.021
				& 0.034 & 0.016 & 0.012 
				& 0.019 $\pm$ 0.008 \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:hyperparameter_2}
\end{table}
\fi
\begin{table}[t!]
	\centering
	\caption{
		Results by varying $(\beta, \tau$) on two tasks, horse $\rightarrow$ zebra and dog $\rightarrow$ dog w/ glasses, using data retrieved from the LAION-5B dataset~\cite{schuhmann2022laion}.
	}
	%\vspace{0.1in}
	%\setlength\tabcolsep{1.7pt} 
	\scalebox{0.75}{
		%\resizebox{\linewidth}{!}{
			\begin{tabular}{c| ccc ccc| cccccc}
				\multirow{2}{*}{($\beta$, $\tau$)} 
				%& \multicolumn{3}{c}{DDIM}
				& \multicolumn{6}{c|}{horse $\rightarrow$ zebra}
				& \multicolumn{6}{c}{dog $\rightarrow$ dog w/ glasses} \\ 
				%& \multicolumn{3}{c}{DDIM}
				& (0.1, 25) & (0.3, 25) & (0.5, 25) & (0.3, 15) & (0.3, 25) & (0.3, 35)
				& (0.6, 25) & (0.8, 25) & (1.0, 25) & (0.8, 15) & (0.8, 25) & (0.8, 35)
				%& \multicolumn{1}{c}{std}
				\\ \hline
				%& \multicolumn{3}{c}{Avg} \\ %\\
				
				%\cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13} \cline{14-16}
				
				%\cline{1-16}
				
				{CS}
				& 0.322 & 0.324	& 0.329
				& 0.332 & 0.324 & 0.300
				% & 0.322 $\pm$ 0.011 \\
				& 0.309 & 0.312	& 0.319
				& 0.317 & 0.312 & 0.307 \\
				% & 0.313 $\pm$ 0.005 \\
				
				{BD}
				& 0.077 & 0.085	& 0.097
				& 0.183 & 0.085 & 0.035 
				% & 0.094 $\pm$  0.049 \\
				& 0.025 & 0.026	& 0.035
				& 0.068 & 0.026 & 0.017 \\
				% & 0.033 $\pm$  0.018 \\
				
				{SD}
				& 0.033 & 0.037	& 0.041
				& 0.065 & 0.037 & 0.020 
				% & 0.039 $\pm$ 0.015 \\
				& 0.015 & 0.016	& 0.021
				& 0.034 & 0.016 & 0.012 \\
				% & 0.019 $\pm$ 0.008 \\
				
				\hline
				%\bottomrule 
			\end{tabular}
			
			%}
	}
	% 
	\label{tab:hyperparameter}
	
\end{table}
%
\begin{figure*}[t!]
	\centering
	%\vspace{-5pt}
	%\vspace{0.2cm}
	\scalebox{1}{
	\includegraphics[width=\linewidth]{./figures/ICCV_Ablation_2row.pdf}}
	%\vspace{-5pt}
	\caption{Qualitative results of the proposed method by varying $\gamma$ on data sampled from the LAION-5B dataset~\cite{schuhmann2022laion}, relying on the pretrained Stable Diffusion~\cite{rombach2022high}. 
		%LAION-5B dataset~\cite{schuhmann2022laion} using the pretrained Stable Diffusion~\cite{rombach2022high}.
		%Comparisons between various values of $\gamma$ in our proposed method. Optimal image quality usually observed at $\gamma=0.2$.
	}
	%Qualitative results of Pix2Pix on the Cityscapes dataset.
	% ``Output" denotes the ground-truth and ``Original" represents the uncompressed generator.}
%\vspace{-1mm}
\label{fig:gamma}
\end{figure*}
%
\iffalse
%
\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{./figures/ECCV_Rebuttal_SimpleLERP.pdf}
	\caption{Qualitative Comparison between PIC and PIC with simple LERP.}
	%Additional qualitative results of the proposed method and other text-driven image-to-image translation methods~\citep{hertz2022prompt, tumanyan2023plug, parmar2023zero} using the pre-trained Stable Diffusion~\citep{rombach2022high} and real images sampled from the LAION 5B dataset~\citep{schuhmann2022laion} on the cat $\rightarrow$ dog task.} 
\label{fig:simplelerp}
\end{figure}
%
\fi


